Search for new phenomena in a lepton plus high jet multiplicity final state with the ATLAS experiment using $\sqrt{s}$ = 13 Tev proton-proton collision data

A search for new phenomena in final states characterized by high jet multiplicity, an isolated lepton (electron or muon) and either zero or at least three $b$-tagged jets is presented. The search uses 36.1 fb$^{-1}$ of $\sqrt{s}$ = 13 TeV proton-proton collision data collected by the ATLAS experiment at the Large Hadron Collider in 2015 and 2016. The dominant sources of background are estimated using parameterized extrapolations, based on observables at medium jet multiplicity, to predict the $b$-tagged jet multiplicity distribution at the higher jet multiplicities used in the search. No significant excess over the Standard Model expectation is observed and 95% confidence-level limits are extracted constraining four simplified models of $R$-parity-violating supersymmetry that feature either gluino or top-squark pair production. The exclusion limits reach as high as 2.1 TeV in gluino mass and 1.2 TeV in top-squark mass in the models considered. In addition, an upper limit is set on the cross-section for Standard Model $t\bar{t}t\bar{t}$ production of 60 fb (6.5 $\times$ the Standard Model prediction) at 95% confidence level. Finally, model-independent limits are set on the contribution from new phenomena to the signal-region yields.

==> event-sel.tex <==
\section{Event Selection}
\label{sec:sel}

Events are selected online using a single electron or muon trigger. For  the analysis selection at least one electron or muon (as defined above) is required in the event.
The analysis is carried out with two sets jet \pT cuts to give sensitivity to a more broad range of models. These cuts are applied to all jets in the event and are \pT $> 40 \GeV$, or \pT $> 60 \GeV$.
The analysis requires at least five jets above the threshold.
It separates events by jet-mutliplicity (for the given \pt threshold) (in bins from 5 to 9 with an additional inclusive '10+ bin) and $b$-jet multiplicity (in bins from 0 to 3 with an additional inclusive 4+ bin).
For probing a specific model all of these bins in data are simulateously fit to extract the expected signal yield, in what is labelled a 'model dependent' fit.
For searching for an unknown BSM model signal regions (SRs) are defined which could be populated by a signal, and where the SM contribution is small. For each jet \pT threshold these signal regions are defined in terms of jet and $b$-jet multiplicity requirements as:
\begin{itemize}
\item $N_{jet}=8, N_{b-jet}=0$
\item $N_{jet}=8, N_{b-jet}>=3$
\item $N_{jet}=9, N_{b-jet}=0$
\item $N_{jet}=9, N_{b-jet}>=3$ 
\item $N_{jet}=10, N_{b-jet}=0$ 
\item $N_{jet}=10, N_{b-jet}>=3$
\end{itemize}
For estimating the backgrounds in these regions only lower $N_{jet}$ bins are used in the fit, and the SR bin is not used.
Due to the efficiency of the $b$-tagging algorithm used, signal models with large $b$-jet multiplicities can have significant contamination in the two $b$-tag bin which can bias the top background estimate reducing the sensitivity of the search. To avoid this the two $b$-tag bin is not included in the fit for the high jet multiplicity slices. Even with this signal contamination in the one b-tag bin can weaken the sensitivity.
(NOTE: could have a table showing the 'discovery' SRs and which CR bins are used for each??)





